Turbine location-aware multi-decadal wind power predictions for Germany using CMIP6

Climate change will impact wind and therefore wind power generation with largely unknown effect and magnitude. Climate models can provide insights and should be used for long-term power planning. In this work we use Gaussian processes to predict power output given wind speeds from a global climate model and compare the aggregated predictions to actual power generation. Analyzing past climate model data supports the use of CMIP6 climate model data for multi-decadal wind power predictions and highlights the importance of being location-aware. Our predictions up to 2050 reveal only minor changes in yearly wind power generation. We find that wind power projections of the two in-between climate scenarios SSP2-4.5 and SSP3-7.0 closely align with actual wind power generation between 2015 and 2023. Our analysis also reveals larger uncertainty associated with Germany's coastal areas in the North as compared to Germany's South, motivating wind power expansion in regions where future wind is likely more reliable. Overall, our results indicate that wind energy will likely remain a reliable energy source in the future.

==> acknowledgements.tex <==
\section*{Acknowledgements}
This study was funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany's Excellence Strategy – EXC number 2064/1 – Project number 390727645 and the Athene Grant of the University of Tübingen. The authors thank the International Max Planck Research School for Intelligent Systems (IMPRS-IS) for supporting Nina Effenberger, and the Natural Sciences and Engineering Research Council of Canada (NSERC) [RGPIN-2020-05783] for supporting Rachel H. White. We acknowledge support by Open Access Publishing Fund of University of Tübingen. Open Access funding enabled and organized by Projekt DEAL. WOA Institution: Eberhard Karls Universitat Tubingen Consortia Name : Projekt DEAL. Nina wants to thank Roland Stull and the Weather Forecast Research Team at UBC for (intellectual) resources!
